Incremental Prompting: Episodic Memory Prompt for Lifelong Event Detection

Lifelong event detection aims to incrementally update a model with new event types and data while retaining the capability on previously learned old types. One critical challenge is that the model would catastrophically forget old types when continually trained on new data. In this paper, we introduce Episodic Memory Prompts (EMP) to explicitly preserve the learned task-specific knowledge. Our method adopts continuous prompt for each task and they are optimized to instruct the model prediction and learn event-specific representation. The EMPs learned in previous tasks are carried along with the model in subsequent tasks, and can serve as a memory module that keeps the old knowledge and transferring to new tasks. Experiment results demonstrate the effectiveness of our method. Furthermore, we also conduct a comprehensive analysis of the new and old event types in lifelong learning.

==> 3approach_backup.tex <==
\section{Approach}

\subsection{Lifelong Event Detection Baseline}
\label{sec:baseline}
\paragraph{Span-based Event Detection}
In this paper, we develop our approach based on a span-based event detection model.
% Similar to (cite), each training instance contains a sentence $w_{1:n}$, a span offset $(s, e)$, and an event type label $y$. 
We first encode the sentence with BERT to obtain the contextual representations $\mathbf{x}_{1:L} = \text{BERT}(x_{1:L})$. Note that we freeze BERT's parameters in our method and all baselines. 
For each span, we concatenate its starting and ending token representations and feed them into a multilayer perceptron (MLP) to get the span representation $\mathbf{h}_{span}$. Then, we apply a linear layer on $\mathbf{h}_{span}$ to predict the type distribution of the span $p^{t}=linear(\mathbf{h}_{span})$, where $t$ denotes the $t$-th task. We use cross-entropy loss to train the model on $\mathcal{D}_t$:
\begin{equation}
\mathcal{L}_{C} = -\sum_{(x^t, (x_i^t, x_j^t),y^t)\in \mathcal{D}_t} \text{log}\ p^{t}.
\end{equation}

% \begin{equation}
% \mathbf{e}_{span} = \text{MLP}_s([\mathbf{h}_s; \mathbf{h}_e]) \\
% \end{equation}
% Then, we apply a linear layer on $\mathbf{h}_{span}$ for prediction. Denote the logits from the model at $t$-th stage as $p^{t}$. We use cross-entropy loss to train the model on the current task:
% \begin{equation}
% \mathcal{L}_{C} = -\sum_{(x, y)\in \mathcal{D}_t} \text{log}\ p^{t}.
% \end{equation}
% The prediction is the event type with the maximum logit value.

\paragraph{Experience Replay} To alleviate the catastrophic forgetting issue, a common strategy is to store a limited amount of data from old types in a memory buffer and replay them in subsequent tasks. Thus, after training on $t$-th task, we apply the herding algorithm~\cite{}\lifu{add reference} to select 20\lifu{how many? for each type or in total}\minqian{solved} training samples for each type into the memory buffer, denoted as $\mathcal{M}$. We use $p^{t}$ to denote the logits predicted by the model at $t$-th stage, so the loss for experience repaly is:
\begin{equation}
\mathcal{L}_{ER} = -\sum_{(x^r, (x_i^r, x_j^r),y^r)\in \mathcal{M}} \text{log}\ p^{t}.
\end{equation}

% Storing a limited amount of data in old types in a memory buffer and replaying them in subsequent tasks has been one of the most common practice in class-incremental learning.
% After training on $t$-th task, we apply the widely used herding algorithm (cite) to select several training samples into the memory buffer, denoted as $\mathcal{M}$. Denote the logits from the model at $t$-th stage as $p^{t}$. The loss for experience repaly is:
% \begin{equation}
% \mathcal{L}_{ER} = -\sum_{(x, y)\in \mathcal{M}} \text{log}\ p^{t}.
% \end{equation}
% We also use cross-entropy loss during experience replay:
% \begin{equation}
% \mathcal{L}_{ER} = - \sum_{(x, y)\in \mathcal{M}} \text{log}\ p^{t}.
% \end{equation}
% (3) we further investigate the effect of reducing the frequency of memory replay.

% \minqian{add exemplar memory balance, as event types are imbalanced}

\paragraph{Knowledge Distillation} As another popular strategy to alleviate the forgetting problem, knowledge distillation (KD) is to ensure the output probabilities from the current and previous model to be matched, and the features encoded by the current model not distorted too much from those learned from the previous model. Following~\cite{cao2020increment}, we apply both \emph{prediction-level} and \emph{feature-level} distillation, and use a temperature parameter to rescale the probabilities of prediction-level KD. Denote the scaled output probability in $t$-th task as $\hat{p}^{t}$. The prediction-level KD loss is computed as:
\begin{equation}
    \mathcal{L}_{PD} = - \sum_{(x^r, (x_i^r, x_j^r),y^r)\in\mathcal{M}} \hat{p}^{t-1}\ \text{log}\  \hat{p}^{t}.
\end{equation}
The feature-level KD loss is:
\begin{equation}
    \mathcal{L}_{FD} = \sum_{(x^r, (x_i^r, x_j^r),y^r)\in\mathcal{M}} 1 - g(\Bar{\mathbf{h}}_{span}^{t-1}, \Bar{\mathbf{h}}_{span}^{t}),
\end{equation}
where $g$ is the cosine similarity function. $\Bar{\mathbf{h}}_{span}^{t-1}$ and $\Bar{\mathbf{h}}_{span}^{t}$ are $l_2$-normalized features from the model at $t-1$ and $t$ stages, respectively.

% Knowledge distillation (KD) is another popular technique for lifelong learning (cite). The key idea of KD in class-incremental learning is that the output probabilities from the current and previous model should be matched, and the feature encoded by the current model should be not distorted too much from that in the previous model. We apply both \emph{prediction-level} and \emph{feature-level} distillation~\cite{cao2020increment} in the baselines. We use a temperature parameter to rescale the probabilities for prediction-level KD. Denote the scaled output probability in $t$-th task as $\hat{p}^{t}$. The prediction-level KD loss is computed as:
% \begin{equation}
%     \mathcal{L}_{PD} = - \sum_{(x,y)\in\mathcal{M}} \hat{p}^{t-1}\ \text{log}\  \hat{p}^{t}.
% \end{equation}
% Denote $g$ as the cosine similarity function. The feature-level KD loss is:
% \begin{equation}
%     \mathcal{L}_{FD} = \sum_{(x,y)\in\mathcal{M}} 1 - g(\Bar{\mathbf{h}}_{span}^{t-1}, \Bar{\mathbf{h}}_{span}^{t}),
% \end{equation}
% where $\Bar{\mathbf{h}}_{span}^{t-1}$ and $\Bar{\mathbf{h}}_{span}^{t}$ are $l_2$-normalized features from the model at $t-1$ and $t$ steps, respectively.


\paragraph{Optimization}
We apply a weighting factor $\lambda$ to control how much loss from experience replay and knowledge distillation to use in each batch. The final loss is computed as:
\begin{equation}
    \mathcal{L} = \mathcal{L}_C + \lambda(\mathcal{L}_{ER}+\mathcal{L}_{PD}+\mathcal{L}_{FD}).
    \label{equa:baseline_train}
\end{equation}

% \minqian{use feature-level and prediction-level distillation during exemplar replay. explain why we did not use distillation on current data: to focus on the effect of exemplar data and replay }

% \subsection{Overall Design}
% show the motivation and the overview on the prompting pipeline

% \subsection{Prompt Design}


\subsection{Episodic Memory Prompting} 

To better overcome the catastrophic forgetting issue and improve the generalizability of event detection method under class-incremental setting, we further design a continuous prompting approach that relies on Episodic Memory Prompts to preserve the knowledge learned from each task and transfer to new tasks.

Given an income task $\mathcal{D}_t$ and its corresponding new event type set $\mathcal{C}_t = \{c_1^t,...,c_{n_t}^t\}$, we first initialize a sequence of new \emph{prompts} $\mathbf{C}^t=[\mathbf{c}_1^t,...,\mathbf{c}_{n_t}^t]$ where $\mathbf{c}_i^t\in\mathbb{R}^{1\times e}$ is a type-specific prompt for type $c_i^t$. $e$ is the embedding dimension size. In our experiments, we use the event type names as the prior knowledge to initialize the parameter of each event type prompt $\mathbf{c}_i^t$ (see Section~\ref{sec:implement} for details). Note that we always preserve the prompts learned from previous tasks, thus the accumulated prompts until the $t$-th task are represented as $\mathbf{I}^t=[\mathbf{C}^1,...,\mathbf{C}^t]$. Given a particular sentence $x_i^t$ from $D^t$, we concatenate the it with the accumulated prompts $\mathbf{I}^t$, encode the whole sequence with the pre-trained language model, e.g., BERT~\cite{}\lifu{cite}, and obtain the sequence of contextual representations $[\tilde{\mathbf{X}}^t_i; \tilde{\mathbf{I}}^t]$, where $\tilde{\mathbf{X}}^t_i$ and $\tilde{\mathbf{I}}^t_i$ denote the sequence of contextual embeddings of $x_i^t$ and $\mathbf{I}^t$ respectively. $[;]$ is concatenation operation. Then, similar as the baseline approach in Section~\ref{sec:baseline}, we will use $\tilde{\mathbf{X}}^t_i$ as the contextual representations to detect events and optimize the model with Equation~\ref{equa:baseline_train}.

% Despite prompting methods' appealing properties for lifelong learning, it is still not clear how to directly use task-specific prompts in \emph{class-incremental} setting, as task boundary is not accessible in inference. 
% Our goal is to learn a unified prompting framework, where prompts can store task-specific knowledge for all-seen tasks, and they can be jointly used in inference without knowing task boundaries. To this end, we develop Episodic Memory Prompt that consists of \emph{task sub-prompts} for each seen task. Different from existing prompting methods that switch the prompts for each different task, our EMP keeps all the learned prompts in the model, such that the acuqired knowledge can be maximally preserved and transferred to new tasks. 

% We first denote the number of event types in the ontology at $t$-th training stage as $n_t$, i.e., $\mathcal{C}_t = \{c_1^t,...,c_{n_t}^t\}$. At each stage, we first initialize a \emph{sub-prompt} for the incoming task, denoted as $\mathbf{C}^t$. The sub-prompt $\mathbf{C}^t$ consists of distinct embeddings for all the event types in this task, i.e., $\mathbf{C}^t=[\mathbf{c}_1^t,...,\mathbf{c}_{n_t}^t]$. In this work, we use a single vector for each type, i.e., $\mathbf{c}_i^t\in\mathbb{R}^{1\times e}$, such that $\mathbf{C}^t\in\mathbb{R}^{n_t\times e}$, where $e$ is the embedding dimension. Here we use the event type names as the event priors to initialize each event embedding $\mathbf{c}_i^t$ (see Section~\ref{sec:implement} for details). Note that we always preserve the prompts learned in previous tasks. Denote the accumulated sub-prompts upon $t$-th stage as $\mathbf{I}^t=[\mathbf{C}^1,...,\mathbf{C}^t]$. We incorporate the accumulated task prompts into the pre-trained language model via modifying the embedding layer: $[\mathbf{X}^t_i; \mathbf{I}^t]$, where $\mathbf{X}^t_i$ is the embeddings of $i$-th instance, $[;]$ is concatenation operation.

At the end of each training stage, we keep the learned prompts from the current task $\mathbf{C}^t$ in the model, and then initialize and incorporate a new prompt $\mathbf{C}^{t+1}$ for the next task incrementally: $\mathbf{I}^{t+1} = [\mathbf{I}^{t};\mathbf{C}^{t+1}]$.
In other words, our EMP can serve as a parameterized episodic memory module that stores the knowledge for each learned type, and transfer the capability acquired from previous tasks to new tasks. %As all previous task-specific knowledge has been explicitly stored in a shared prompt, our approach does not require a task identity to indicate which prompts to use. 
% \begin{equation}
% % \small
% \mathbf{x}_{\text{[CLS]}} \; \mathbf{x}_{1}\; ...\; \mathbf{x}_{L}\; \mathbf{x}_{\text{[SEP]}}\; \mathbf{C}^t \;  \text{[SEP]}
% \label{eq:input}
% \end{equation}
% It is worth noting that we select a relatively "weak" prior to initialize prompts as we want to demonstrate that our framework does not rely too much on human prior knowledge. We will investigate how to incorporate stronger prior knowledge into our EMPs in the future work. 





% In addition to adapting the old knowledge to new tasks, we also want to transfer the new knowledge in old tasks, as some of old and new types are related . However, if we directly update the learned prompts in following tasks, we cannot guarantee the prompts maintain previous task-specific knowledge. To address this issue, we apply an additional supervision signal to optimize EMP, such that it can continue to learn a event-specific representation during new-to-old knowledge transfer. 

% While we have addressed the major challenge in adapting prompts in class-incremental learning, there still remains an issue: we use trainable soft prompts in our EMP so that the model is more expressive and adaptable, as discrete templates require considerable engineering and tend to be suboptimal. Also, as 

% After we initialize the prompt parameters, remaining challenge: prompts are still task-agnostic without an explicit objective to update. needs to directly apply supervised signal to each prompts: from implicit update to explicit update and assign the prompts with more explicit meaning

\paragraph{Entangled Prompt Optimization} We expect the EMPs to be specific to the corresponding event types and preserve the knowledge of each event type from previous tasks. To achieve this goal, we design an entangled prompt optimization strategy. Specifically, after obtaining the contextual representations of the sentence as $\tilde{\mathbf{X}}^t_i$ and EMPs as $\tilde{\mathbf{I}}^t_i$, for each span we get the span representation $\tilde{\mathbf{h}}_{span}$. Then we entangle the span features with event type specific prompts by computing an event type probability distribution over all prompts: $p_c = \text{MLP}(\tilde{\mathbf{I}}^t_i)\cdot\tilde{\mathbf{h}}_{span}$.

after the EMP is encoded from the language model, we first apply a MLP layer to further encode the prompt.
Then, we apply dot product between the encoded prompts $\mathbf{H}_{prom}$ and the span representation $\mathbf{h}_{span}$ to obtain the \emph{prompt logits}: $p_c = \mathbf{H}_{prom}^{T}\mathbf{h}_{span}$.
% In other words, we can consider the encoded prompts as another classification layer. 
Finally, we combine the original logits and the \emph{prompt logits} to get the final logits for prediction in our framework: $p_{sum} = p + p_c$.

% Specifically, after the EMP is encoded from the language model, we first apply a MLP layer to further encode the prompt.
% Then, we apply dot product between the encoded prompts $\mathbf{H}_{prom}$ and the span representation $\mathbf{h}_{span}$ to obtain the \emph{prompt logits}: $p_c = \mathbf{H}_{prom}^{T}\mathbf{h}_{span}$.
% % In other words, we can consider the encoded prompts as another classification layer. 
% Finally, we combine the original logits and the \emph{prompt logits} to get the final logits for prediction in our framework: $p_{sum} = p + p_c$.

% The motivation of this mixture-of-expert style classification is that: (1) the decisions from two different sources can enhance each other and make the final decision better; (2) by classifying the spans with prompts, the prompt parameters in the input layer can be optimized in a more explicit way comparing to previous prompting frameworks where prompts can only be optimized implicitly.\minqian{how to better illustrate the motivation of adding the two logits?}

% \subsection{Optimization}
% \minqian{add optimization loss. optional: show training algorithm}

==> 4experiment_backup.tex <==
\section{Experiments}
\subsection{Experiment Settings}

\paragraph{Class-incremental Dataset Construction} We use two datasets for the experiments. (1) ACE05-EN contains 33 event types with 597 documents and 5,311 mentions. (2) MAVEN contains 168 event types in the general domain with 3,623 documents and 96,987 mentions. For both ACE and MAVEN, we follow the \emph{oracle negative} setting in~\cite{yu2021lifelong} and construct the class-incremental dataset as follows. We divided the ontology into 5 subsets, with no overlapping event types between any two of them. These 5 subsets then constitute a sequence of 5 tasks denoted as $\mathcal{D}_{1:5}$. We use the same partition and task order permutations in \cite{yu2021lifelong}\footnote{\lifu{add one sentence to talk about the motivation of permutation}}. 


% \paragraph{Dataset} We use two datasets for the experiments. (1) ACE05-EN contains 33 event types with 597 documents and 5,311 mentions. (2) MAVEN contains 168 event types in the general domain with 3,623 documents and 96,987 mentions. For both ACE and MAVEN, we follow the dataset setup in~\cite{yu2021lifelong} and evaluate all our experiments in the \emph{oracle negative} setting proposed by them.
% % We use the original development set as the test set and randomly collect another development set from the training data. 
% % It's worth noting that we make sure the development set covers all event types.

% \paragraph{Class-incremental Dataset Construction} 
% For both ACE and MAVEN datasets, we construct the class-incremental dataset as follows. We divided the ontology into 5 subsets, with no overlapping event types between any two of them. These 5 subsets then constitute a sequence of 5 tasks denoted as $\mathcal{D}_{1:5}$. We use the same partition and task order permutations in \cite{yu2021lifelong}. 
% The distribution of event types in subsets is shown in Table~\ref{tab:distribution}.

% \subsection{Experiment Settings}

% \paragraph{Oracle Negative}
% The \emph{oracle negative} setting is proposed by~\cite{yu2021lifelong}, where the \emph{oracle negative} instances include all negative instances in the original dataset and all unlearned event types. To simulate the situation of adding the new types' annotations, we exclude instances for learned types when training the model on new types. We report the results in the oracle negative setting in both ACE and MAVEN dataset. 
% We mainly use the oracle negative setting for our discussions. 

% \noindent\textbf{Silver Negative}

\paragraph{Evaluation}
We use micro F1 score as our primary evaluation metric. During the learning process from $\mathcal{D}_1$ to $\mathcal{D}_5$, we constantly test the model on the entire test set (which contains the whole ontology) and take the mentions of unseen event types as negative instances.

\paragraph{Implementation Details}
\label{sec:implement}
We use AdamW~\cite{adamw} optimizer during training with learning rate set to $1e-4$ and weight decay set to $1e-2$. Different from previous work~\cite{yu2021lifelong}, we set the batch size to 1 as we encode each sentence once and consider all target spans in the sentence at the same time. We adopt gradient accumulation with the step set to 8. As the number of batches is large, we apply a periodic replay strategy with the interval set to 10 to reduce computational cost. For each class-incremental task $\mathcal{D}_{t}$, we set the maximum number of training epochs to 20. We adopt the early stopping strategy with patience 5, i.e., the training stops if the performance on the development set does not increase for 5 epochs. We set the weighting factor $\lambda=k/(s+k)$, where $s$ is the number of predicted spans and $k$ is set to 50. 

The parameters of each prompt in EMPs are initialized with the corresponding event type name. Specifically, there are three cases in the initialization: (1) If the type name is \emph{single-token} and it is contained in BERT's vocabulary, we directly use the pre-trained embedding of this token to initialize the prompt; (2) If the type name is \emph{multiple-token} and the tokens are contained in BERT's vocabulary, we take the average of the pre-trained embeddings of these tokens to initialize the prompt; (3) If the type name contains \emph{Out-of-Vocabulary (OOV)} tokens, we replace the OOV tokens with the synonyms that are contained in BERT's vocabulary. 

\begin{table*}[!htbp]
	\centering
	\resizebox{0.95\textwidth}{!}
	{
	\begin{tabular}{l | ccccc | ccccc}
    \toprule
    & \multicolumn{5}{c}{MAVEN}  & \multicolumn{5}{c}{ACE05-EN} \\
    \midrule
    Task &1 &2 & 3 & 4 & 5 & 1 &2 & 3 & 4 & 5  \\ 
    \midrule
    BERT-ED & 63.51 & 39.99 & 33.36 & 23.83 & 22.69 & 58.30 & 43.96 & 38.02 & 21.53 & 25.71 \\
    iCaRL*~\cite{icarl} & 18.08 & 27.03 & 30.78 & 31.26 & 29.77 & 4.05 & 5.41 & 7.25 & 6.94 & 8.94 \\
    EEIL~\cite{eeil} & 63.51 & 50.62 & 45.16 & 41.39 & 38.34 & 58.30 & 54.93 & 52.72 & 45.18 & 41.95 \\
    BIC~\cite{bic} & 63.51 & 46.69 & 39.15 & 31.69 & 30.47 & 58.30 & 45.73 & 43.28 & 35.70 & 30.80 \\
    KCN~\cite{cao2020increment} & 63.51 & 51.17 & 46.80 & 38.72 & 38.58 & 58.30 & 54.71 & 52.88 & 44.93 & 41.10 \\
    KT~\cite{yu2021lifelong} & 63.51 & 52.36 & 47.24 & 39.51 & 39.34 & 58.30 & \textbf{55.41} & 53.95 & 45.00 & 42.62 \\
    \midrule
    EMP (Ours) &\textbf{67.62} & \textbf{58.33} & \textbf{54.53} & \textbf{47.70} & \textbf{44.30} & \textbf{59.60} & 53.19 & \textbf{55.20} & \textbf{45.64} & \textbf{43.28} \\
    \midrule
    % Upperbound (Origin) & / & / & / & / & 64.50 & / & / & / & / & 67.78 \\
    Upperbound (Ours) & / & / & / & / & 66.68 & / & / & / & / & 68.22 \\
    % GP+Tune TP (Ours) & 70.52 & 58.70 & \textbf{57.39} & 51.06 & 26.86 \\ 
    % GP+Fix TP (Ours) & 70.76 & \textbf{60.19} & 55.69 & 42.42 & 27.01 \\
    % GP+Fix TP\&MLP (Ours) & 70.35 & 58.76 & 57.04 & 44.78 & 24.35 \\
    \bottomrule
    \end{tabular}
	} 
	\caption{Comparison between our approach and baselines in terms of micro F-1 (\%) on 5 class-incremental tasks. We report the averaged results on 5 permutations of tasks to alleviate the affect of task order.}
	\label{tab:main}
\end{table*}

\paragraph{Baselines} We consider the following baselines for comparison: (1) \textbf{BERT-ED}: simply trains the BERT based event detection model on new tasks without prompts, experience replay or knowledge distillation. It's the same as the span-based event detection baseline in Section~\ref{sec:baseline}. (2) \textbf{KCN}~\cite{cao2020increment}: as the original approach studied a different setting, we adapt their hierarchical distillation as the baseline\lifu{use one sentence to describe this approach}. (3) \textbf{KT}~\cite{yu2021lifelong}: transfer knowledge between old types and new types in two directions. (4) \textbf{Upperbound}: trains the same model on all types in the datasets jointly. We present the details of \textbf{iCaRL}~\cite{icarl}, \textbf{EEIL}~\cite{eeil}, and \textbf{BIC}~\cite{bic} in Appendix.\minqian{TODO} 
For fair comparison, our approach and all baselines (except for the Upperbound baseline) are built upon \textbf{KCN} and use the same experience replay and knowledge distillation strategies described in Section~\ref{sec_emp}.

\subsection{Results}

We present the main results in Table~\ref{tab:main}. Note that as iCaRL does not use experience replay strategy and is not affected by the modification, we report the result in~\cite{yu2021lifelong} for reference. Based on Table~\ref{tab:main}, we have following observations: (1) by comparing the performance of various approaches on Task 1 which are not affected by any catastrophic forgetting, our prompting based approach improves 4.1\% F-score on MAVEN and 1.3\% F-score on ACE05, demonstrating that by incorporating task-specific prompts, event detection itself can be significantly improved. EMPs even provide more improvement on MAVEN which contains a lot more event types than ACE05, which shows the potential of incorporating EMPs for fine-grained event detection; (2) \textbf{KCN} can be viewed as an ablated version of our approach without the EMPs. Our approach consistently outperforms \textbf{KCN} on almost all tasks on both datasets, demonstrating the benefit of EMPs on improving the generalizability of event detection under class-incremental setting and addressing the catastrophic forgetting problem; (3) By comparing XX and XX, we see XX, \lifu{complete it} which verifies that experience replay and knowledge distillation can dramatically alleviate the catastrophic forgetting problem. (4) Comparing with the upperbound performance, there is still a large gap between the current lifelong learning approaches and the upperbound, indicating that catastrophic forgetting still remains a very challenging problem. 

It is worth noting that either storing too many data or replaying the examples too frequently will increase the computational burden, and more critically, deteriorate the value of lifelong learning research. We thus constrain that only one exemplar instance is allowed to use in each training batch, compared with~\newcite{yu2021lifelong} that appends the whole memory set to each training batch. Therefore, most results in our paper cannot be directly compared with the results reported in~\cite{yu2021lifelong}.
%(4) Our approach \lifu{pointing that our approach achieves more improvement on MAVEN, demonstrating that EMPs can also work well or even betterr for fine-grained event detection}

%Our method improves around 4\% F1 in Task 1 because our EMP not only improve the lifelong learning but also event detection itself. For MAVEN, our method outperforms all the considered baselines, and the performance gain consistently larger than the margin in Task 1. For ACE, our method also achieves promising improvement on all tasks but Task 2. The reason why the improvement is not as large as that on MAVEN could be the difference in prompt length. Since we use a prompt for each event type, the prompts used in MAVEN is much longer than that in ACE. This indicates prompting methods might be very sensitive to prompt length.

%It is worth noting that either storing too many data or replaying the examples too frequently will increase the computational burden, and more critically, deteriorate the value of lifelong learning research. We thus constrain that only one exemplar instance is allowed to use in each training batch, compared with the previous work~\cite{yu2021lifelong} that appends the whole memory set to each training batch. Therefore, most results in our paper cannot be directly compared with the results reported in~\cite{yu2021lifelong}.

% We also report the upperbound performance in Table~\ref{tab:main}. There is still a large gap between current lifelong learning techniques and the upperbound, which indicates catatrophic forgetting still remains as a very challenging problem. 

% significant improve on MAVEN; ACE only improved marginally: prompt size might be too small; leave increasing or more dynamic prompting in future
% \minqian{how to explain EEIL is better, and BIC is worse, compared to Pengfei's paper?}



% \begin{table}[!htbp]
% 	\caption{Comparison between our approach and baselines in terms of micro F-1 (\%) on 5 incremental tasks on ACE under oracle negative setting. }
% 	\centering
% 	\resizebox{0.5\textwidth}{!}
% 	{
% 		\begin{tabular}{l | ccccc}
%     \toprule
%     Task &1 &2 & 3 & 4 & 5  \\ 

%     \bottomrule
%     \end{tabular}

% 	} 
% 	\label{tab:comp}
% \end{table}

% \begin{table}[!htbp]
% 	\caption{Results in the setting without exemplar replay and knowledge distillation on 5 incremental tasks on MAVEN.}
% 	\centering
% 	\resizebox{0.5\textwidth}{!}
% 	{
% 		\begin{tabular}{l | ccccc}
%     \toprule
%     Task &1 &2 & 3 & 4 & 5  \\ 
%     \midrule
%     Origin & 67.44 & 41.29 & 35.00 & 22.51 & 21.85 \\
%     EMP (Ours) & \textbf{70.57} & \textbf{43.42} & \textbf{36.95} & \textbf{25.55} & \textbf{23.24} \\

%     \bottomrule
%     \end{tabular}

% 	} 
% 	\label{tab:comp}
% \end{table}
